Solving SAT and MaxSAT with a Quantum Annealer: Foundations, Encodings, and Preliminary Results

Quantum annealers (QAs) are specialized quantum computers that minimize objective functions over discrete variables by physically exploiting quantum effects. Current QA platforms allow for the optimization of quadratic objectives defined over binary variables (qubits), also known as Ising problems. In the last decade, QA systems as implemented by D-Wave have scaled with Moore-like growth. Current architectures provide 2048 sparsely-connected qubits, and continued exponential growth is anticipated, together with increased connectivity. We explore the feasibility of such architectures for solving SAT and MaxSAT problems as QA systems scale. We develop techniques for effectively encoding SAT -and, with some limitations, MaxSAT- into Ising problems compatible with sparse QA architectures. We provide the theoretical foundations for this mapping, and present encoding techniques that combine offline Satisfiability and Optimization Modulo Theories with on-the-fly placement and routing. Preliminary empirical tests on a current generation 2048-qubit D-Wave system support the feasibility of the approach for certain SAT and MaxSAT problems.

==> background_pf.tex <==
We represent Boolean values $\set{\bot, \top}$ as the binary values $\set{-1,
1}$ respectively.
%
Consider $G\defas\tuple{V,E}$ as usual 
and a Boolean formula $F(\xs)$ over a set of Boolean
variables \xs, and assume each $x_i$ is mapped univocally into a vertex
in $V$. 
Then a {\em penalty function} $\Px$ is defined as in \eqref{eq:penfunction}:

\begin{align}
  \label{eq:penfunction}
\Px \defas \offset{} + \sum_{i\in V} \theta_i x_i + \sum_{(i,j) \in E}
\theta_{ij} x_i x_j,
\\
  \text{such that }\quad  \forall \xs\  P_F(\xs| \ts)
  \begin{cases}
= 0 &\text{ if }   F(\xs)=\top \\
   \geq g_{min} &\text{ if } F(\xs)=\bot.
  \end{cases}\label{eq:pencriteria}
\end{align}
%The penalty function $P_F(\xs| \ts)$ is a polynomial over the rationals where:
%
\begin{itemize}
\item $V$ and $E$ are the vertices and
edges of the hardware graph (see e.g. Figure~\ref{fig:chimera}). 

\item The $x_i$s are binary variables in $\set{-1,1}$, 
each associated to one vertex in $V$, which represent qubits values
  that are set by the annealing process.

\item The $\ts$ parameters are rationals values which are set by the
  user before each quantum-annealing run, s.t.
  $\offset{} \in\ ]-\infty,+\infty[$ (\emph{offset}) is added to guarantee
  $\Px\ge 0$, 
  each $\theta_i \in [-2,2]$ (\emph{bias}) is associated to the qubit
  $x_i$ in $V$, and 
  each $\theta_{ij} \in [-1,1]$ (\emph{coupling}) is associated to an
  edge in $E$.
  
  

\item $g_{min}$ is a strictly-positive rational value, which allows for
  discriminating models from counter-models. In general, we would like
  it to be as
  big as possible.
  %% In practice the appropriate value for this parameter changes
  %% according performance of the quantum annealer.
\end{itemize}

%% There are three kinds of $\ts$ parameters:

%% \begin{itemize}
%% \item $\offset{}$ is called \emph{offset} and it is an unbounded rational.
%% \item $\theta_i$ values are called \emph{biases}. They are rational values in the interval
%%   $[-2,2]$. There is a bias parameter associated to each vertex in the qubits
%%   graph of Figure \ref{fig:chimera}.
%% \item $\theta_{ij}$ values are called \emph{couplings}. They are in the interval
%%   $[-1,1]$. They can be set only for pairs of qubits that are connected by an
%%   edge in the qubit graph (again, see Figure \ref{fig:chimera}).
%% \end{itemize}


Then the \emph{SAT-2-QUBO encoding problem} is described as follows:
\emph{given \Fx, find an injective map from \xs to $V$ and proper
values for the $\ts$'s in \eqref{eq:penfunction} so that
$\Px$ satisfy  \eqref{eq:pencriteria}.}
%
%% Our problem is the following: \uline{given \Fx, find the values of $\ts$ so that
%% $\Px$ satisfy the previous criteria \eqref{eq:pencriteria}}.
%
The resulting values of the $\ts$'s can be fed to the QA, which 
finds a set of
$x$ values that minimize $\Px$. By \eqref{eq:pencriteria}, if such value
is zero, then $x$ satisfies $F$. 
%
\begin{example}
\label{es:exampleiff}
  The equivalence between two variables,
  $\Fx\defas (x_1 \leftrightarrow
  x_2)$, can be represented with a single
  coupling: $\offset{} = 1, \theta_1 = \theta_2 =
  0, \theta_{12} = -1$, that is, $\Px \defas 1 - x_1x_2$, where
  $g_{min}=2$. In fact, $\Px=0$ if $x_1,x_2$ have the same value,
  $\Px=2$ otherwise.
\end{example}



\begin{example}\label{es:exampleand}
  The and function, $\Fx\defas x_3 \leftrightarrow
  (x_1 \wedge x_2)$, when $x_1,\ x_2,\ x_3$ are placed into a triangle, 
  can be represented by
  $
  \offset{} = \frac{3}{2},\ \theta_1 = \theta_2 = -\frac{1}{2},\
  \theta_3 = 1,\ \theta_{12} = \frac{1}{2},\ \theta_{13} = \theta_{23}
  = -1
  $
  That is, $\Px = \frac{3}{2} -\frac{1}{2} x_1 - \frac{1}{2}x_2 + x_3 +\frac{1}{2}x_1 x_2 - x_1
x_3 - x_2 x_3 $, where
  $g_{min}=2$. In fact, $\Px=0$ if $x_1,x_2$ have the same value,
  $\Px=2$ otherwise.
Again the constraints are respected, with $g_{min} = 2$, as shown in
following table:
\begin{center}
$
 \begin{array}{|l|r|r|r|r|r|r|r|r|} \hline
 x_1 & -1& -1& -1& -1&  1&  1&  1& \ \ 1 \\
 x_2 & -1& -1&  1&  1& -1& -1&  1&  1 \\
 x_3 & -1&  1& -1&  1& -1&  1& -1&  1 \\
 \hline
 \Px & 0 & 6& 0& 2& 0& 2& 2& 0 \\
 \hline
 \end{array}
$
\end{center}
%
%% \begin{center}
%%   \begin{tabular}{|c|c|c|c|}
%%     \hline
%%     $x_1$ & $x_2$ & $x_3$ & $P_F(\xs)$ \\
%%     \hline
%%     -1 & -1 & -1 & 0 \\
%%     \hline
%%     -1 & -1 & 1 & 6 \\
%%     \hline
%%     -1 & 1 & -1 & 0 \\
%%     \hline
%%    -1 &  1 & 1 & 2 \\
%%     \hline
%%     1 & -1 & -1 & 0 \\
%%     \hline
%%     1 & -1 & 1 & 2 \\
%%     \hline
%%     1 & 1 & -1 & 2 \\
%%     \hline
%%    1 &  1 & 1 & 0 \\
%%     \hline
%%   \end{tabular}
%%   \end{center}
\end{example}



\begin{IGNORE}
\begin{example}\label{es:exampleiff}
  The equivalence between two variables, $\Fx\defas x_1 \leftrightarrow
  x_2$ can be represented with a single
  coupling:
  $$\offset{} = 1 \quad \theta_1 = \theta_2 = 0 \quad \theta_{12} = -1$$.
  These parameter settings give us the function:
$$\Px = 1 - x_1x_2$$.
The constraints are respected, with $g_{min}=2$:
\begin{center}
  \begin{tabular}{|c|c|c|}
    \hline
    $x_1$ & $x_2$ & $P_F(\xs)$ \\
    \hline
    -1 & -1 & 0 \\
    \hline
    -1 & 1 & 2 \\
    \hline
    1 & -1 & 2 \\
    \hline
    1 & 1 & 0 \\
    \hline
  \end{tabular}
\end{center}
\end{example}
\end{IGNORE}

\begin{IGNORE}
\begin{example}\label{es:exampleand}
  The binary AND function, $ x_3 \leftrightarrow
  (x_1 \wedge x_2)$ can be represented by three qubits in a triangle
   in this way:

  $$\offset{} = \frac{3}{2} \quad \theta_1 = \theta_2 = -\frac{1}{2} \quad
  \theta_3 = 1 \quad \theta_{12} = \frac{1}{2} \quad \theta_{13} = \theta_{23}
  = -1$$
  That is, $P_F = \frac{3}{2} -\frac{1}{2} x_1 - \frac{1}{2}x_2 + x_3 +\frac{1}{2}x_1 x_2 - x_1
x_3 - x_2 x_3 $.
Again the constraints are respected, with $g_{min} = 2$:
\begin{center}
  \begin{tabular}{|c|c|c|c|}
    \hline
    $x_1$ & $x_2$ & $x_3$ & $P_F(\xs)$ \\
    \hline
    -1 & -1 & -1 & 0 \\
    \hline
    -1 & -1 & 1 & 6 \\
    \hline
    -1 & 1 & -1 & 0 \\
    \hline
   -1 &  1 & 1 & 2 \\
    \hline
    1 & -1 & -1 & 0 \\
    \hline
    1 & -1 & 1 & 2 \\
    \hline
    1 & 1 & -1 & 2 \\
    \hline
   1 &  1 & 1 & 0 \\
    \hline
  \end{tabular}
  \end{center}
\end{example}
\end{IGNORE}


==> boolean-matching.tex <==
Boolean matching is the task of checking NPN equivalence
  between Boolean functions. It is used to search the library for adequate gate
  representations of components of a formula. It has an exponential worst case
  complexity, but is very quick for small-sized functions and not a
  limiting factor in the encoding process. It has been extensively been studied
  (see \cite{soeken2016heuristic,Hinsberger:1998:BML:277044.277100,correia2001classifying}).


==> computing.tex <==
As stated before, the most sensible approach to the encoding problem
is to pre-compute a library of encoded Boolean functions and decompose
the input problem instance into a set of these functions.

%\subsection{A General schema}

Regarding research question \ref{qs:apply-qa}, a general schema of the
encoding and annealing process is shown in Figure
\ref{procgraph}. This is not the only possible method (see
\cite{dridi2016prime,choi2011different}) but it is the most efficient
so far for SAT and constraint satisfaction problems. The whole process
can be grouped in two phases. In the \emph{offline phase}, the gates
library is populated with efficient representations of commonly used
Boolean functions to provide a library of modular (occupying 1, 2 or 4
Chimera tiles) gates. The offline phase can be the most
computationally-expensive part, but is performed only once and can be
performed with no time constraints with large clusters. The online
phase has performance constraints and must be performed in the
shortest time possible. In the online phase, the input problem is
processed and fed to the QA to obtain the solution. The input problem
is first minimized, then it is decomposed and converted into a set of
QUBO problems, which are conjoined into a Chimera-like Ising model by
placement and routing. The Ising model is fed to the quantum annealer,
which returns a solution for the original SAT problem.

\begin{figure*}[tb]
  \centering{
\begin{adjustbox}{max width=0.9\textwidth}

  \begin{tikzpicture}[
    every node/.style={inner sep=1em, align=center},
    every edge/.append style={->, thick},
    datum/.style={fill=white, rounded rectangle,draw},
    oper/.style={rectangle, fill=gray!20, rounded corners, draw},
    db/.style={cylinder, cylinder uses custom fill,
      cylinder body fill=yellow!50,
      cylinder end fill=yellow!50,
      shape border rotate=90,
      aspect=0.25, draw},
    mach/.style={parallelepiped, draw=white, fill=black, text=white}]

\node [oper] (synth) {Decomposition \\ and mapping};
\node [oper] (bmatch) [above=of synth] {Boolean \\ matching};
\node [db] (library) [above=of bmatch] {Library};
\node [oper] (minim) [left= of synth] {Minimization};
\node [datum] (satp) [left=of minim]  {SAT \\ problem};
\node [oper] (encoding) [left=of library]{pre-encoding};
\node [datum] (boolf) [left=of encoding, align=center] {Boolean \\ functions};
\node [datum] (qubo) [right=of synth, align=center] {QUBO \\ problem};
\node [oper] (placeroute) [right=of qubo, align=center] {Placement \\ and routing};
\node [datum] (isingm) [right=of placeroute, align=center] {Ising \\ model};
\node [mach] (dwave) [right=of isingm, align=center] {D-Wave \\ QA};
\node [datum] (sol) [right= of dwave] {Solution};

\path (boolf) edge (encoding);
\path (encoding) edge (library);
\path (library) edge (bmatch);
\path (bmatch) edge (synth);
\path (synth) edge (bmatch);
\path (satp) edge (minim);
\path (minim) edge (synth);
\path (synth) edge (qubo);
\path (qubo) edge (placeroute);
\path (placeroute) edge (isingm);
\path (isingm) edge (dwave);
\path (dwave) edge  (sol);

\begin{scope}[on background layer]
  \node [fill=yellow!30, fit=(boolf) (encoding), inner ysep= 1.2em] (box) {};
  \node [anchor=south] [below=-2em of box] {Offline process};
  \node [fill=green!30, fit=(minim) (bmatch) (dwave)] (box2) {};
  \node [anchor=north] [above=-2em of box2] {On-the-fly process};
\end{scope}

\end{tikzpicture}
\end{adjustbox}}
\caption{Graph of the encoding process. \label{procgraph}}
\end{figure*}

Not every component of the picture is a potential target for improvement. Some
tasks will not be subject to research on my behalf, as the available techniques
work sufficiently well.
In particular:

\begin{itemize}
\item Boolean formula minimization consists in
simplifying the input formula to reduce its size in terms of its graph
representation (generally AIGs). This is a pretty mature field on its own
 \cite{Mishchenko06dag-awareaig,mishchenko2005fraigs}.

\item Boolean matching is essentially the task of checking NPN equivalence
  between Boolean functions. It is used to search the library for adequate gate
  representations of components of a formula. It has an exponential worst case
  complexity, but is very quick for small-sized functions and definitely not a
  limiting factor in the encoding process. It has been extensively been studied
  (see \cite{soeken2016heuristic,Hinsberger:1998:BML:277044.277100,correia2001classifying}).
\end{itemize}

\paragraph{Library pre-encoding}
We want to find effective encodings of selected Boolean functions to add to our
library. While performing this task we can afford to use large computing
resources and a longer execution time, as it can be completed ahead-of-time and
is not dependent on the problem input. In section 2 we asked (in research
question \ref{qs:minimal-ising}) how to obtain the minimum Ising model for a
formula, and in section 3 we presented the SMT-based encoding method
\cite{bian2014discrete}. Regarding this method, he current state of the art may
be improved considering alternatives to the SMT formulation.


An idea would be to tackle the quantified variables in \eqref{eq:encoding1} with
\emph{binary decision diagrams} (BDDs). Binary decision diagrams are efficient
data structures that enable complete representations of binary
functions \cite{DBLP:journals/csur/Bryant92}.
\iffalse
This data structure consist in a directed acyclic graph where each node is
associated with a Boolean variables. Each node represent a decision on its
variable assignment: it has two outbound edges, one leading to the sub-BDD
representing the formula after assigning $\bot$ and one leading to the sub-BDD
for the opposite $\top$ decision. Each path of a diagram represents an
assignment that leads to one of two special nodes: the $\top$ node and the
$\bot$ node, depending on whether the assignment satisfies the formula or not.
\fi
BDD grow exponentially in size in the worst case, but record all possible truth
values of a represented function. This is useful to handle the quantified binary
variables of \eqref{eq:encoding1}. By using SMT techniques during the
construction of the BDD on the quantified variables, we may be able to avoid the
space explosion associated with direct quantifier elimination.

\paragraph{SMT-based positioning}
Another idea is to further investigate the use of SMT solvers to find the best
variable placements on the constrained Chimera topology \cite{rsebanote}.
State-of-the-art SMT-based encoding assumes that variables are
associated with a fixed position on the Chimera tile, whereas topology constraints
are the most constraining for the feasibility of an encoding.
A better idea would be to search all legal qubit graphs for the smallest encoding.
Topology information (about which coupling is available and which is forced to
be 0) expressed in the SMT formula can be separated from variable order in the
Boolean formula through the use of uninterpreted functions.

We can add a new injective mapping $p(\xs)$ between Boolean variables and binary variables
as in \eqref{penfunctionpos}.
When the placement $p(\xs)$ is represented as uninterpreted functions in the SMT
formula, we can let the SMT solver decide the best positions.
Furthermore, we can exploit the highly-symmetric nature of the Chimera
architecture to reduce the search space (see \cite{sakallah2009symmetry,rsebanote}).

\begin{align}
  \label{penfunctionpos}
P_F(\xs|\ts, p(\xs)) \triangleq \offset{} + \sum_{i\in V} \theta_i p(x_i) + \sum_{(i,j) \in E}
\theta_{ij} p(x_i) p(x_j)
\end{align}

The challenge is to efficiently port the variable
elimination optimization to this version, as it relies heavily on the fixed
variable position on the qubit graph.

\paragraph{Decomposition and mapping}
The decomposition and mapping phase is the one where the input Boolean formula
is decomposed into functions that are stored in the library. This part is
related to research question \ref{qs:decomposition}. It is critical to use as
few functions as possible to exploit as much as possible the efficient
pre-computed library. The synthesis part so far has always been performed
naively: given a set of constraints over the variable, each constraint is found
in the library and mapped. The only improvement on it has been the
pre-processing step presented in the fault analysis paper
\cite{bian2014discrete}. Various advanced techniques have been devised in the
digital logic synthesis literature. These work on a different set of assumptions
but they can be adapted to the SAT encoding problem.

For example, the literature on \emph{technology mapping} can be useful to identify the
best decomposition of the SAT formula according to the circumstances. Technology
mapping is the process of mapping a technology-independent circuit
representation to the physical gates used in a digital circuit
\cite{mishchenko2005technology,een2007applying}.
Usually technology mapping is used to reduce circuit delay and load, and
performs minimization as a further step. For the context of QA
we do not have issues about delay and load, though minimization is important because
reducing the number of nodes helps in placement and routing.
The success of these techniques vary on the size and the quality of the library
gate, the cost function used, and so on. I plan to experiment with these
parameters in order to further optimize the workflow for the QA encoding
problem.

Another interesting concept that might be brought from digital logic synthesis
is \emph{rewiring} \cite{chang1999circuit}. As is it possible to reconfigure a
logic circuit in order to remove wires that are too hard to place, it may be
possible to modify the structure of a QUBO problem when the embedding is
unfeasible for some particular chain.

\paragraph{Placement and routing}
In the placement and routing phase, the input is a QUBO polynomial that
generally respects the penalty function constraint apart from topology. In this
part, embedding algorithms are used to build chains and obtain a Ising model
with a correct qubit graph. This task is related to research question
\ref{qs:embedding}.

The placement and routing step is the bottleneck for the current state of the
art. Improving the previous step can simplify the problem but the
place-and-route algorithms themselves may have margins for improvement. The
digital logic literature is not as useful here considering the special
characteristics of the hardware.
My plan for this part is to revisit the best algorithms available and try to customize
them in order to optimize speed and exploit the flexibility of the previous
steps.

An interesting idea would be to use SAT and SMT based techniques. A customized SMT
formulation of the placement and routing problem would allow us to obtain a
complete algorithm that is able to ensure the existence or absence a solution.
%,but a naive SMT-based encoding of the embedding problem is not efficient. 


==> experimental_maxsat2.tex <==
%% \newcommand{\SI}[2]{#1 #2}
%% \newcommand{\micro}{\ensuremath{\mu}}
%% \newcommand{\second}{\ensuremath{s}}

\subsubsection{Weighted MaxSAT sampling}
One of the strengths of D-Wave's QA hardware is its ability to rapidly sample the near-optimal solutions: current machines typically anneal at a rate of \SI{10}{\micro\second} or \SI{20}{\micro\second} per sample and are designed to take thousands of samples during each programming cycle. As a result it is likely that the first practical benefits of QA will come from applications which require many solutions rather than a single optimum. 

Another important consideration in solving SAT instances using QA is that the QA hardware cannot be made aware of the optimality of solution; for example, QA cannot terminate when all clauses in a SAT problem are satisfied. In this way, QA hardware behaves more like an inexact MaxSAT solver than SAT solver.

To demonstrate the performance of QA in this regime, we have generated
MaxSAT instances which have many distinct optimal solutions, and
compared the performance of inexact MaxSAT solvers in rapidly
generating those solutions. These problems were generated from the
2-in-4-SAT instances described above by removing a fraction of the constraints and then adding constraints on single variables with smaller weight.


\begin{table}[t]
\begin{center}
\subtable[\label{table:maxsat_firstsol}]{
\begin{tabular}{|l|r|r|}
\hline
\multicolumn{3}{|c|}{\textbf{D-Wave 2000X}}\\\hline
\textbf{Problem size}&\textbf{\# solved}&\textbf{\% correct}\\\hline
\textbf{32 vars}&100&78.7\\\hline
\textbf{36 vars}&100&69\\\hline
\textbf{40 vars}&100&60.2\\\hline
\textbf{44 vars}&100&49.9\\\hline
\textbf{48 vars}&100&40.4\\\hline
\textbf{52 vars}&100&35.2\\\hline
\textbf{56 vars}&100&24.3\\\hline
\textbf{60 vars}&100&22.3\\\hline
\textbf{64 vars}&99&17.6\\\hline
\textbf{68 vars}&99&13\\\hline
\textbf{72 vars}&98&9.6\\\hline
\textbf{76 vars}&94&6.6\\\hline
\textbf{80 vars}&93&4.3\\\hline
\end{tabular}}
\qquad
\subtable[\label{table:maxsat_firstsol_timing}]{
\begin{tabular}{|l|r|r|r|r|}
\hline
\multicolumn{5}{|c|}{\textbf{MaxSAT solvers: avg time (ms)}}\\\hline
\textbf{Problem size}&\textbf{g2wsat}&\textbf{rots}&\textbf{maxwalksat}&\textbf{novelty}\\\hline
\textbf{32 vars}&0.02&0.018&0.034&0.039\\\hline
\textbf{36 vars}&0.025&0.022&0.043&0.06\\\hline
\textbf{40 vars}&0.039&0.029&0.056&0.119\\\hline
\textbf{44 vars}&0.049&0.043&0.07&0.187\\\hline
\textbf{48 vars}&0.069&0.054&0.093&0.311\\\hline
\textbf{52 vars}&0.122&0.075&0.115&0.687\\\hline
\textbf{56 vars}&0.181&0.112&0.156&1.319\\\hline
\textbf{60 vars}&0.261&0.13&0.167&1.884\\\hline
\textbf{64 vars}&0.527&0.159&0.207&4.272\\\hline
\textbf{68 vars}&0.652&0.21&0.27&8.739\\\hline
\textbf{72 vars}&0.838&0.287&0.312&14.118\\\hline
\textbf{76 vars}&1.223&0.382&0.396&18.916\\\hline
\textbf{80 vars}&1.426&0.485&0.43&95.057\\\hline
\end{tabular}} 
\caption{\label{table:maxsat}%
(a) Number of problem instances (out of 100) solved by the QA hardware using 100 samples, and average fraction of samples from the QA hardware that are optimal solutions. Annealing was executed at a rate of \SI{10}{\micro\second} per sample, for a total of \SI{1}{\milli\second} of anneal time per instance. (b) Time in \SI{}{\milli\second} taken to find an optimal solution by various inexact weighted MaxSAT solvers, averaged over 100 MaxSAT instances of each problem size. Classical computations were performed on an Intel i7 2.90GHz $\times$ 4 processor. gw2sat\ignoreinshort{ \cite{li2005g2wsat}}, rots\ignoreinshort{ \cite{smyth2003rots}}, and novelty\ignoreinshort{ \cite{mcallester1997novelty}} are as implemented in ubc-sat \cite{tompkins_ubcsat:_2004}. All classical algorithms are performed with the optimal target weight specified; in the absence of a target weight they are much slower. }
\end{center}
%\end{table}
%
%\vspace{-1.0cm}
%\begin{table}
\begin{center}
\subtable[\label{table:maxsat_cutoff_dw}]{
\begin{tabular}{|l|r|r|}
\hline
\multicolumn{3}{|c|}{\textbf{D-Wave 2000X}}\\\hline
\textbf{Size}&\textbf{anneal only}&\textbf{wall-clock}\\\hline
\textbf{32 vars}&448.5&443.9\\\hline
\textbf{36 vars}&607&579.9\\\hline
\textbf{40 vars}&1007.9&922\\\hline
\textbf{44 vars}&1322.6&1066.6\\\hline
\textbf{48 vars}&1555.4&1111.8\\\hline
\textbf{52 vars}&3229&1512.5\\\hline
\textbf{56 vars}&2418.9&1147.4\\\hline
\textbf{60 vars}&4015.3&1359.3\\\hline
\textbf{64 vars}&6692.6&1339.1\\\hline
\textbf{68 vars}&6504.2&1097.1\\\hline
\textbf{72 vars}&3707.6&731.7\\\hline
\textbf{76 vars}&2490.3&474.2\\\hline
\textbf{80 vars}&1439.4&332.7\\\hline
\end{tabular}}
\qquad
\subtable[\label{table:maxsat_cutoff_classical}]{
\begin{tabular}{|l|r|r|r|r|}
\hline
\multicolumn{5}{|c|}{\textbf{MaxSAT solvers}}\\\hline
\textbf{Size} &\textbf{g2wsat}&\textbf{rots}&\textbf{maxwalksat}&\textbf{novelty}\\\hline
\textbf{32 vars}&448.5&448.5&448.5&448.5\\\hline
\textbf{36 vars}&607&606.9&606.9&606.8\\\hline
\textbf{40 vars}&1007.7&1006.3&1005.3&1005\\\hline
\textbf{44 vars}&1313.8&1307.1&1311.7&1255.5\\\hline
\textbf{48 vars}&1515.4&1510.7&1504.9&1320.5\\\hline
\textbf{52 vars}&2707.5&2813&2854.6&1616.2\\\hline
\textbf{56 vars}&2021.9&2106.2&2186.6&969.8\\\hline
\textbf{60 vars}&2845.6&3061.7&3289&904.4\\\hline
\textbf{64 vars}&3100&4171&4770&570.6\\\hline
\textbf{68 vars}&2742.2&3823.3&4592.4&354.8\\\hline
\textbf{72 vars}&1841.1&2400.2&2943.4&212.6\\\hline
\textbf{76 vars}&1262.5&1716&2059.2&116.4\\\hline
\textbf{80 vars}&772.2&1111.1&1363.9&66.7\\\hline
\end{tabular}}
\caption{\label{table:maxsat_numsols}%
Number of distinct optimal solutions found in 1 second by various MaxSAT solvers, averaged across 100 instances of each problem size. (a) ``anneal only" accounts for only the \SI{10}{\micro\second} per sample anneal time used by the D-Wave processor. ``wall-clock" accounts for all time used by the D-Wave processor, including programming and readout. (b) Classical computations were performed as in Table \ref{table:maxsat_firstsol_timing}.}
\end{center}
\end{table}

\begin{IGNOREINSHORT}
The instances were generated as follows: 
\begin{enumerate}
\item Beginning with the 2-in-4-SAT instances of the previous section, we remove one of the partitions of the variable set, and change one 2-in-4 constraint to 1-in-4. (This makes the SAT problem unsatisfiable: for an $n$ variable problem, the first partition demands exactly $n/2$ true variables, while the second demands exactly $n/2-1$.)
\item We change the SAT problem into a weighted MaxSAT problem by assigning existing constraints a weight of 3 and randomly assign each variable or its negation a soft weight of weight 1.
\item We repeated generate MaxSAT instances of this form, until we find an instance in the the optimal solution has exactly one violated clause of weight 3; at least $n/3$ violates clauses of weight 1, and at least $200$ distinct optimal solutions.
\end{enumerate}
\end{IGNOREINSHORT}

Table \ref{table:maxsat} summarizes the performance of the D-Wave hardware and other inexact MaxSAT solvers in generating a single optimal solution, while Table \ref{table:maxsat_numsols} considers generating distinct optimal solutions. For each solver and problem size, the latter table indicates the number of distinct solutions found in 1 second, averaged across 100 problem instances of that size. For the smallest problems, 1 second is sufficient for all solvers to generate all solutions. For larger problems, the QA hardware generates more solutions, provided we consider only time spent annealing and not time spent programming the hardware and reading out solutions.

%Table \ref{table:maxsat} summarizes the performance of the D-Wave hardware and other inexact MaxSAT solvers in generating a single optimal solution. As in Section \ref{sec:sat-exper}, it is difficult and perhaps unfair to compare performance directly; however Table \ref{table:maxsat_firstsol_timing} shows the time to find an optimal solution for classical solvers, while Table \ref{table:maxsat_firstsol} shows the number of instances solved by the QA hardware by taking 100 samples, which corresponds to \SI{1}{\milli\second} of annealing. 


==> foundations.tex <==
We introduce first some notation, conventions and terminology we adopt
in this paper: 
% Hereafter we represent Boolean values $\set{\bot, \top}$ as the binary values $\set{-1,
% 1}$.
% %
% In what follows,
\begin{itemize}
\item
$G\defas\tuple{V,E}$ is the Chimera hardware graph, as in \sref{sec:background_qa};
\item
Boolean values $\set{\bot, \top}$ are represented as the binary values $\set{-1,
1}$;
\item
\Fx is a Boolean function on a set of {\em input Boolean
variables} $\xs\defas\set{x_1,...,x_n}$;
%, s.t.   $n\defas |\xs|$;
\item
 $\as\defas\set{a_1,...,a_h}$
 is a set of {\em ancillary Boolean variables} (``{\em ancillas}'');
 %, s.t.  $h\defas|\as|$;
\item
% $\zs\defas\xs\cup\as=\set{z_1,...,z_{n+h},...}$
 $\zs\defas\set{z_1,...,z_{n+h},...,z_{|V|}}$
 is a set of Boolean variables which are associated to each
 node in $V$. 
 %
\ignore{
\item
$\offset{}\in (-\infty,+\infty)$ (``{\em offset}''),
$\theta_i \in [-2,2]$ (``{\em biases}') and
$\theta_{ij} \in [-1,1]$ (``{\em couplings}''),
s.t. $z_i,z_j\in\zs$,
and $g_{min}>0$ (``{\em gap}'')
are rational-valued parameters.~%
\footnote{%
Notationally, since we are representing non-direct graphs, we are
assuming a strict 
ordering in the $z$'s so that only one between $\theta_{z_iz_j}$ and
$\theta_{z_jz_i}$ exists, and no $\theta_{z_iz_i}$ exists.}
%% \item
%% $g_{min}>0$ is the {\em gap} of $F$.%
%% ~\footnote{The notation \g is due to the fact that the value depends on
%% both $F$ and $|\as|$ (and also on the ranges \rangeb and \rangec, which we consider
%% fixed for now).}
%
}
\end{itemize}
%
\ignore{
We assume each $z_i\in\zs$ is mapped univocally into a vertex
in $V$; with a little abuse of notation,
we say that $z_i\in V$ and $(z_i,z_j)\in E$, i.e., 
$z_i,z_j$ implicitly denote the nodes
where they are mapped into.
}
%


==> intro.tex <==
\TODO{Add paragraph on ``The quest for quantum computing''\\}
\TODO{Add paragraph on SAT \& hard problems\\}


Quantum Annealing (QA) is a specialized form of computation that uses
quantum mechanical effects to efficiently sample low-energy
configurations of particular cost functions on binary
variables. Currently, the largest QA system heuristically minimizes an
Ising cost function given by
\begin{eqnarray}
  \label{eq:isingmodel}
  E(\zs) &\defas & \sum_{i \in V} \DWbiasi z_i +
                   \sum_{\substack{(i,j)\in E}} \DWcoupij{} z_i z_j
  \\
  \label{eq:isingmodel_minimization}
  && \argmin_{\zs \in \set{-1,1}^{|V|}} E(\zs).
\end{eqnarray}
where $G=(V,E)$ is an undirected graph of allowed variable interactions.  Ising
models are equivalent to \emph{Quadratic Unconstrained Binary
  Optimization} (QUBO) problems, which use $\{0,1\}$-valued
variables rather than $\pm 1$-valued variables.  \footnote{The
  transformation between $z_i\in\set{-1,1}$ and $x_i\in\{0,1\}$ is
  $z_i = 2x_i-1$.}  The decision version of
the Ising problem on most graphs $G$ is NP-complete.

Theory suggests that quantum annealing may solve some optimization
problems faster than state-of-the-art algorithms
\cite{farhi2001quantum}.  Quantum effects such as tunneling and
superposition provide QA with novel mechanisms for escaping local
minima, thereby potentially avoiding suboptimal solutions commonly
found by classical algorithms based on bit-flip operations (such as
WalkSAT).  Practical QA systems are not guaranteed to return optimal
solutions; however, the D-Wave processor has been shown to outperform
a range of classical algorithms on certain problems designed to match
its hardware structure \cite{denchev16google,king17fcl}. These results
also provide guidance about the kinds of energy landscapes on which QA
is expected to perform well.

Our ultimate goal is to exploit QA as an engine for solving SAT
and other NP-hard problem instances which are relatively small
but hard enough to be out of the reach of state-of-the-art solvers
(e.g., SAT problems coming from cryptanalysis).
\emph{SAT} is the problem of deciding the satisfiability of arbitrary
formulas on atomic propositions, typically written in conjunctive
normal form.  \emph{MaxSAT} is an optimization extension of SAT, in
which each clause is given a positive penalty if the clause is not
satisfied, and an assignment minimizing the sum of the penalties is
sought.
\ignoreinshort{ Efficient SAT and MaxSAT tools are widely available \cite{HandbookOfSAT2009}.}


\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\columnwidth]{chimera3x3.pdf}
  \caption{\label{chimera}
    Example of the Chimera topology: the hardware graph for system
    of 72 qubits in a 3-by-3 grid of tiles. (D-Wave 2000Q systems
    have 2048 qubits in a 16-by-16 grid.)
%\RSCOMMENT{Content of caption moved to intro text.}
\ignore{
    This topology consists of a lattice of strongly-connected
    components of 8 qubits, called \emph{tiles}. Each tile consists of
    a complete bipartite graph between two sets of four qubits. One
    set, the ``vertical" set, is connected to the tiles above and
    below; the other set, the ``horizontal" set, is connected to the
    tiles to the left and to the right. Notice that each qubit is
    connected with at most six other qubits. In other words, each
    variable $z_i$ in the Ising model \eqref{eq:isingmodel} has at
    most $6$ non-zero $\DWcoupij{}$ interactions with other
    variables.}}
\end{figure}

% Hereafter, if not specified otherwise, we
% assume that the graph $G$ is the 2048-qubit hardware
% graph of the D-Wave 2000Q machine, that is, the $16\times 16$-tile
% extension of the graph in Figure~\ref{chimera}.
%% figures positioned on the top require less space

\begin{IGNOREINLONG}
In principle, converting SAT to optimization of an Ising cost function
is straightforward. However, practical QA systems such as the D-Wave
2000Q  offer  sparse connectivity between
variables. The connectivity graph $G$ of current D-Wave
processors is shown in Figure~\ref{chimera}, and is called the
\emph{Chimera} graph.
Further, because the Ising model is solved on a physical, analog
device, it is subject to engineering limitations. The D-Wave 2000Q
system currently requires $\DWbiasi \in [-2,2]$ and
$\DWcoupij{} \in [-1,1]$ and there are limits on the precision to
which these parameters may be specified.  Parameter imprecisions
act as small additive noise sources on parameter values, and arise
from operating quantum mechanical systems in real-world
environments. These real-world practicalities necessitate a carefully
defined SAT-to-Ising encoding.
\end{IGNOREINLONG}
\begin{IGNOREINSHORT}
\input{qa_detail}
\end{IGNOREINSHORT}

These practical constraints generate a challenging problem
because the SAT encoding must be done both {\em effectively}
(i.e., in a way that uses only the limited number of qubits and
connections available within the QA architecture, while optimizing
performance of the QA algorithm), and {\em efficiently} (i.e., using
a limited computational budget for computing the encoding).
In this paper, we formalize this problem and provide practical
algorithms.

A direct formulation of the encoding problem results in a large system of linear
inequalities over continuous- and Boolean-valued variables.  This system
can be effectively addressed with Satisfiability or Optimization Modulo
Theory (SMT/OMT) \cite{barrettsst09,sebastiani15_optimathsat} solvers.
\emph{Satisfiability Modulo the Theory of Linear Rational Arithmetic
  (\smtlarat)} \cite{barrettsst09} is the problem of deciding the
satisfiability of arbitrary formulas on atomic propositions and
constraints in linear arithmetic over the rationals.
\emph{Optimization Modulo the Theory of Linear Rational Arithmetic
  (\omtlarat)} \cite{sebastiani15_optimathsat} extends \smtlarat by
searching solutions which optimize some \larat objective(s).
Efficient \omlarat solvers like \optimathsat \cite{st_cav15} allow for
handling formulas with thousands of Bool\-ean and rational variables
\cite{sebastiani15_optimathsat}.

This monolithic linear programming
approach to encoding typically requires the introduction of
%\ignoreinshort{(possibly many)}
additional
ancillary Boolean variables, and the resultant SMT/OMT problem may be
computationally harder than the original problem.
\ignoreinshort{Also, the number of additional variables may grow
  drastically with the size of the formula encod.}
In contrast, a large Boolean formula can be scalably converted into an Ising model by decomposing it into subformulae, converting
each subformula into an Ising model (perhaps with introduction of additional
fresh variables), and linking variables from different
subformulae. Unfortunately, in practice this decomposition-based
approach requires many auxiliary variables and
connections, which are incompatible with the sparse connectivity restrictions imposed by
 QA architectures.

To cope with these difficulties, we propose a mixed approach, which
combines (i) novel SMT/OMT-based techniques to produce off-line
encodings of commonly-used Boolean subfunctions, with (ii) the usage
of function instantiation and placement-and-routing techniques to
combine and place on-the-fly the encoded functionalities within the QA
architecture.

We have implemented prototype encoders on top of the SMT/OMT tool
%\mathsatfive \cite{mathsat5_tacas13} and
\optimathsat
\cite{st_cav15}. %\RSTODO{possibly rewrite according to the results.}
As a proof of concept, we present some preliminary
empirical evaluation, in which we have executed encoded
SAT and MaxSAT problems on a \linebreak D-Wave~2000Q system.
% against s.o.a. SAT/MaxSAT tools.
%
Although preliminary, the results confirm the feasibility of the
approach.
%
\begin{ADDED}
We stress the fact that this paper is not supposed to present a comparison with
respect to state-of-the-art of classic computing. Rather, this is
intended as a preliminary assessment of the challenges and
potential of QA to impact SAT and MaxSAT solving.
\end{ADDED}

%\textbf{[Summarize all the sections of the paper]}
%\ignoreinshort{
\added{
The rest of the paper is organized as follows.
Section \ref{sec:foundations} presents the theoretical foundations of this work;
Section \ref{sec:computing} describes our mixed approach to cope with this
problem;
\ignoreinshort{Section \ref{sec:related} summarizes the related work;}
Section \ref{sec:expaval} presents a preliminary empirical evaluation;
Section \ref{sec:future} hints future developments.
}
\ignoreinlong{A longer and more detailed version of this paper,
  \added{including a section that describes related work,} is available online
\cite{bian17_frocos17extended}.}


==> penalty2.tex <==
\begin{IGNORE}
We represent Boolean values $\set{\bot, \top}$ as the binary values $\set{-1,
1}$.
%
In what follows,
\begin{itemize}
\item
$G\defas\tuple{V,E}$ is the Chimera HW graph as in \sref{sec:background_qa};
\item
\Fx is a Boolean function on a set of {\em input Boolean
variables} $\xs\defas\set{x_1,...,x_n}$;
%, s.t.   $n\defas |\xs|$;
\item
 $\as\defas\set{a_1,...,a_h}$
 is a set of {\em ancillary Boolean variables} (``{\em ancillas}'');
 %, s.t.  $h\defas|\as|$;
\item
 $\zs\defas\xs\cup\as=\set{z_1,...,z_{n+h}}$
 denotes the set of variables in \xs and \as, without distinction
 between input and ancilla variables.
 %
\item
$\offset{}\in (-\infty,+\infty)$ (``{\em offset}''),
$\theta_i \in [-2,2]$ (``{\em biases}') and
$\theta_{ij} \in [-1,1]$ (``{\em couplings}''),
s.t. $z_i,z_j\in\zs$,
and $g_{min}>0$ (``{\em gap}'')
are rational-valued parameters.~%
\footnote{%
Notationally, since we are representing non-direct graphs, we are
assuming a strict 
ordering in the $z$'s so that only one between $\theta_{z_iz_j}$ and
$\theta_{z_jz_i}$ exists, and no $\theta_{z_iz_i}$ exists.}
%% \item
%% $g_{min}>0$ is the {\em gap} of $F$.%
%% ~\footnote{The notation \g is due to the fact that the value depends on
%% both $F$ and $|\as|$ (and also on the ranges \rangeb and \rangec, which we consider
%% fixed for now).}
%
\end{itemize}
%
We assume each $z_i\in\zs$ is mapped univocally into a vertex
in $V$; with a little abuse of notation,
we say that $z_i\in V$ and $(z_i,z_j)\in E$, i.e., 
$z_i,z_j$ implicitly denote the nodes
where they are mapped into.  
\end{IGNORE}

%\RSTODO{FRO NOW ON STILL UNDER REWRITING\\}
We introduce a set of ancillary variables (``ancillas'')
$\as\defas\set{a_1,...,a_h}$. 
%
We assume each variable in $\xs\cup\as$ is embedded univocally into 
one of the variables $\zs$ associated to vertexes in $V$.
(With a little abuse of notation, we say 
``$z_i\in \xs\cup\as$'' meaning that $z_i$ is in the subset of $\zs$  
onto which the variables in $\xs\cup\as$ are embedded.)
%
We define a {\em penalty function} $\Pxa$  as:
%
\begin{align}
  \label{eq:penfunction}
\Pxa \defas \offset{} + \sum_{\substack{z_i\in \xs\cup\as\\z_i\in V}} \theta_{i} z_i +
\sum_{\substack{z_i,z_j\in \xs\cup\as\\(z_i,z_j) \in E,\ i<j}}
\theta_{ij} z_i z_j,
\\
  \text{such that }\quad  \forall \xs\ \ min_{\set{\as}} \Pxa
  \begin{cases}
= 0 &\text{ if }   F(\xs)=\top \\
   \geq g_{min} &\text{ if } F(\xs)=\bot.
  \end{cases}\label{eq:pencriteria}
\end{align}
where $\offset{}\in (-\infty,+\infty)$ (``{\em offset}''),
$\theta_i \in [-2,2]$ (``{\em biases}') and
$\theta_{ij} \in [-1,1]$ (``{\em couplings}''),
s.t. $z_i,z_j\in\zs$,
and $g_{min}>0$ (``{\em gap}'')
are rational-valued parameters.~%



We call $\Pxa$ ax {\em exact  penalty function} if and only if it verifies a
stronger version of \eqref{eq:pencriteria} in which 
the condition ``$\geq g_{min}$'' is substituted with ``$= g_{min}$''.
%
\ignore{
\eqref{eq:pencriteria} 
\begin{align}
  \text{such that }\quad  \forall \xs\ \ min_{\set{\as}} \Pxa
  \begin{cases}
= 0 &\text{ if }   F(\xs)=\top \\
   = g_{min} &\text{ if } F(\xs)=\bot.
  \end{cases}\label{eq:pencriteria}
\end{align}
}
\noindent
(When $\as=\emptyset$, we denote the penalty function by $\Px$.)
%\RSTODO{Add strict version for MaxSAT.}

The $z_i$s (i.e. the $x_i$s and $a_i$s)
are binary variables in $\set{-1,1}$, 
each associated to one vertex in $V$, which represent qubits values
  that are set by the annealing process.
%
%\item
The $\ts$s are rational values which are set by the
user before each quantum-annealing run.
Notice that the rightmost sum \eqref{eq:penfunction}
implicitly says that $\theta_{ij}=0$ when $(z_i,z_j) \not\in E$. 
%
%\item
$g_{min}$ is a strictly-positive rational value, which allows for
  discriminating models from counter-models.
  In general, it is desirable 
  it to be as
  big as possible for making the process less noise-sensitive.
%\end{itemize}



Then the \emph{SAT-2-QUBO encoding problem} is described as follows:
\emph{given \Fx and $\as$, and given an injective embedding
 from $\xs\cup\as$ into the \zs, find proper
values for the $\ts$'s in \eqref{eq:penfunction} so that
$\Pxa$ satisfy  \eqref{eq:pencriteria} which maximize $g_{min}$.}
%
%% Our problem is the following: \uline{given \Fx, find the values of $\ts$ so that
%% $\Px$ satisfy the previous criteria \eqref{eq:pencriteria}}.

The resulting values of the $\ts$'s can be fed to the QA, which 
searches a set of values of
$\xs,\as$  that minimize $\Pxa$. By \eqref{eq:pencriteria}, if the returned
value of \Pxa is zero, then $\xs$ satisfies $F$.
%
In principle, if the QA where guaranteed to always find a minimum
solution within the sampling time, then we could also conclude that,
if the value of $\Pxa\ge g_{min}$, then $\xs$ falsifies $F$.
In practice, since this is not the case in general, the whole process
cannot certify the unsatisfiablity of a formula. 

%
\begin{example}
\label{es:exampleiff}
  The equivalence between two variables,
  $\Fx\defas (x_1 \leftrightarrow
  x_2)$, can be encoded without ancillas by means of a single
  coupling between two connected vertices, with zero biases: 
%% \ignore{$\offset{} = 1, \theta_1 = \theta_2 =
%%   0, \theta_{12} = -1$, that is, }
$\Px \defas 1 - x_1x_2$, so that
  $g_{min}=2$. In fact, $\Px=0$ if $x_1,x_2$ have the same value,
  $\Px=2$ otherwise.
 Notice that \Px is also an exact penalty function.
\end{example}

The ancilla variables are needed because
ancilla-free encodings are often not possible
within the Chimera HW graph or even with a completely connected graph, 
as shown in the following examples. 

\begin{example}\label{es:exampleand}
  Consider the AND function $\Fx\defas x_3 \leftrightarrow
  (x_1 \wedge x_2)$.
  If $x_1,\ x_2,\ x_3$ could be all connected in a 3-clique,
  then \Fx could be encoded without ancillas by setting
  %% $
  %% \offset{} = \frac{7}{2},\ \theta_1 = \theta_2 = -\frac{1}{2},\
  %% \theta_3 = 1,\ \theta_{12} = \frac{1}{2},\ \theta_{13} = \theta_{23}
  %% = -1
  %% $, 
  %% that is, 
$\Px = \frac{3}{2} -\frac{1}{2} x_1 - \frac{1}{2}x_2 + x_3 +\frac{1}{2}x_1 x_2 - x_1
x_3 - x_2 x_3 $, so that 
  $g_{min}=2$.
\ignoreinshort{
  In fact, %it is easy to see that
  $\Px=0$ if $x_1,x_2,x_3$
  verify \Fx, $\Px=6$ if $x_1=x_2=-1$ and $x_3=1$,
  $\Px=2$ otherwise.
}
%
Unfortunately, the Chimera graph has no cliques, so that
the above AND function needs (at least) one ancilla $a$ to be encoded  as:
$\Pxa =  \frac{5}{2} - \frac{1}{2} x_1 - \frac{1}{2} x_2 + x_3 + \frac{1}{2}
x_1 x_2 - x_1 x_3 - x_2a - x_3a $, which still has gap $g_{min} =2$ and is embedded as in figure
~\ref{fig:mappings_and}.

%
%% \begin{IGNORE}
%% Again the constraints are respected, with $g_{min} = 2$, as shown in
%% following table:
%% %
%% \begin{center}
%% $
%%  \begin{array}{|l|r|r|r|r|r|r|r|r|} \hline
%%  x_1 & -1& -1& -1& -1&  1&  1&  1& \ \ 1 \\
%%  x_2 & -1& -1&  1&  1& -1& -1&  1&  1 \\
%%  x_3 & -1&  1& -1&  1& -1&  1& -1&  1 \\
%%  \hline
%%  \Px & 0 & 6& 0& 2& 0& 2& 2& 0 \\
%%  \hline
%%  \end{array}
%% $
%% \end{center}
%% \end{IGNORE}
%
\end{example}
\begin{figure}[t]
\subfigure[\label{fig:mappings_and}$x_3 \iff (x_1 \wedge x_2)$ with one ancilla.]%
{\includegraphics[width=0.21\columnwidth]{andgraph.pdf} 
}
\subfigure[\label{fig:mappings_xor}$x_3 \iff (x_1 \oplus x_2)$ with three ancillas]%
{\includegraphics[width=0.21\columnwidth]{xorgraph.pdf}\ \ \ \ \ }
\subfigure[\label{fig:mappings_two}$x_4 \iff (x_3 \wedge (x_1 \oplus x_2))$   \hspace{\textwidth}  obtained by combining \ref{fig:mappings_xor} and \ref{fig:mappings_and}.]%
{\includegraphics[width=0.5\columnwidth]{two.pdf}\ \ \ \ \ }
\caption{\label{fig:mappings} Mappings within the Chimera HW graph. \ref{fig:mappings_two} combines \ref{fig:mappings_and} and \ref{fig:mappings_xor} using chained proxy variables. The resulting penalty function encodes the equisatisfiable formula: 
$(y \iff (x_1 \wedge x_2))\wedge (y' \iff y)) \wedge (x_4 \iff (x_3 \wedge y'))$
\TODO{Labels inside nodes?(nodes are small to fit text, could move $x_1$ $x_3$ and $x_4$ to unused qbits instead to be tidier) Labels for ancillas?}}
\end{figure}

\begin{example}
\label{es:examplexor}
Consider the XOR function 
$\Fx\defas x_3 \leftrightarrow (x_1 \oplus x_2)$. Even within a
3-clique, \Fx has no ancilla-free encoding. 
Within the Chimera graph, \Fx
can be encoded with three ancillas $a_1, a_2, a_3$ as:
  $
  \Pxa = 5 + x_3 + a_2 - a_3 + x_1 a_1  - x_1 a_2 - x_1 a_3 - x_2 a_1 - x_2 a_2 
  - x_2 a_3 + x_3 a_2 - x_3 a_3
  $, which has gap $g_{min} = 2$ and is embedded as in figure ~\ref{fig:mappings_xor}.
\end{example}



==> problem2.tex <==
We aim at using D-Wave's QAs as backend engines for solving SAT
and MaxSAT problems. The main intuitions are as follows.

For SAT: 
given a generic Boolean formula $\Fx$,
%  on some input Boolean variables 
% $\xs\defas\set{x_1,...,x_n}$,
% we represent Boolean values $\set{\bot, \top}$ as the binary values
% $\set{-1,1}$ and 
we want to build %from \Fx 
an Ising model
\eqref{eq:isingmodel} to feed to the QA, so that
any minimum-energy value $E(\zs)$ %returned by the QA 
which solves the minimization problem \eqref{eq:isingmodel_minimization}
allows for stating if \Fx is satisfiable or not
 ---and, if yes,
 the value of \zs can be mapped back into a satisfying truth assignment for \Fx.

For MaxSAT: given a set \Fx of clauses each with some positive
penalty, we want to build %from \Fx 
an Ising model
\eqref{eq:isingmodel} to feed to the QA so that
any minimum-energy value $E(\zs)$ %returned by the QA 
which solves the minimization problem \eqref{eq:isingmodel_minimization}
% such that any solution 
% $E(\zs)$  to the minimization problem 
% \eqref{eq:isingmodel_minimization}
represents 
the minimum penalty and \zs can be mapped back 
into one truth assignment minimizing such penalty· 

%
In both cases, to build the Ising model \eqref{eq:isingmodel}
 we need performing two main steps:
\begin{description}
\item[Embedding:] find an injective map from the input variables \xs 
(plus possibly other ancillary variables \as, see below) 
to the qubits \zs of the hardware architecture.
\item[Encoding:] provide proper values for the \DWbiasi{} and
  \DWcoupij{} parameters in \eqref{eq:isingmodel}.
\end{description}

%We remark a few facts. 
In general, the problem of finding an Ising model for \Fx 
presents some remarkable
theoretical and practical difficulties. 


\ignore{
First, for SAT
there must be a 
gap between the energy values of $E(z)$ representing satisfying assignments 
and those representing unsatisfying ones, which is sufficiently big to
be always able to discriminate between the two cases, even in presence
of noise; 

for MaxSAT, the gaps between the minimum-penalty assignments and the
second-best ones should be big enough to discriminate between the them.
}

First, for SAT \resp{MaxSAT}, the gaps between the energy values of $E(z)$
representing satisfying \resp{minimum-penalty} assignments and those
representing unsatisfying \resp{non-minimums-penalty} ones should
% always 
be big enough
to discriminate between the two cases, even in presence of noise.

Second, for any given embedding from $\xs$ into $\zs$, the encoding
problem is typically over-constrained. In fact, the Ising model
\eqref{eq:isingmodel} has to discriminate between $O(2^n)$ satisfying
\resp{minimum-penalty} assignments and $O(2^n)$ other assignments,
whereas the number of degrees of freedom is given by the number of the
\DWbiasi{} and \DWcoupij{} parameters, which in the Chimera
architecture grows as $O(n)$.


\ignore{
- issue of gap
- verify essential properties (compositional)
- overconstrained
}


==> problems_otherissues.tex <==
\paragraph{Multiple-step decomposition} The encoding process explained until now
is meant to convert the entire problem into a single model to be annealed. The
size of the model is fixed for a single machine and depends on the technological
advancements in manufacturing. Thus, we want to know what to do when the problem
we want to solve is still too big to fit into the machine.

There is the need to decompose the problem into smaller sub-problems in order to
allow the use multiple quantum annealing steps. There is no way to pass quantum
information between steps, so the single step result must provide useful
information with an incomplete problem representation.

\paragraph{Disabled qubits} An important problem is that D-Wave's quantum
annealer may have \emph{disabled qubits}. A few qubits on the chip may have
manufacturing defects and be unusable. In this case, we need an embedding method
that is flexible enough to route around such defects. A really efficient
embedding method, able to achieve high utilization on all qubits of a perfect
Chimera architecture, may have difficulties when handling random defects. It is
possible also to simulate in software missing qubits, but then we have to accept
the performance losses.

\paragraph{Noise tolerance} Finally, D-Wave's machine is susceptible to noise.
Interaction with the external environment results in a qubit losing a quantum
state and choosing a random binary value. In this case the annealer may return
non-optimal solutions.

We want to design a process that is robust to noise. In a sense, the machine can
be seen as an incomplete SAT solver that may return imperfect results. Even if
the simplest solution is to run the QA until the value returned satisfies our
formula, imperfect results may still be useful to determine the desired result.



==> problems_sat2qubo.tex <==
Unfortunately, the encoding problem defined
in \sref{sec:penalty} is in general an over-constrained problem.
%
%Given the previous definitions, some issues arise in the encoding process.
First, only few Boolean formulas can be expressed directly as  QUBOs
as in \eqref{eq:penfunction}. 

\begin{example}
\label{es:examplexor}
The
$\Fx\defas x_3 \leftrightarrow (x_1 \oplus x_2)$ has no QUBO direct
encoding as in \eqref{eq:penfunction}.
\end{example}

Second, the Chimera graph is very sparse and has no cliques,
so many direct encodings are often not possible within the Chimera Graph.

\begin{example}
  The and function of Example~\ref{es:exampleand}
  requires a 3-clique,
whereas the current hardware has no such connections, so that
it cannot be directly encoded as in \eqref{eq:penfunction}.
\end{example}



To avoid these problems, our first possible solution is to add \emph{ancillary
  variables}, denoted as $\as$. Ancillary variables, or ancillas, behave as
normal Boolean variables, but we impose looser requirements on them. We extend
penalty function with ancillas in the following way: 
%
\begin{eqnarray}
%\nonumber
\label{eq:penfunction_withancillas}
\Pxa \defas  \offset{}+\sum \theta_i x_i+\sum \theta_{ij} x_i x_j+
  \sum \theta_i a_i+\sum \theta_{ij} a_i x_j+\sum \theta_{ij} a_i a_j
\end{eqnarray}
%
%% \begin{multline}
%%   \Pxa \triangleq \quad  \offset{}+\sum \theta_i x_i+\sum \theta_{ij} x_i x_j +\\
%%   \sum \theta_i a_i+\sum \theta_{ij} a_i x_j+\sum \theta_{ij} a_i a_j
%% \end{multline}
\noi
s.t. both original variables \xs and ancillas \as are mapped into
qubits in $V$.


Ancillas allow us to reformulate the SAT-2-QUBO encoding problem
of \sref{sec:penalty}
as follows:
\emph{given \Fx and \as, find an injective map from \xs and \as to $V$
and proper values for the $\ts$'s
in \eqref{eq:penfunction_withancillas} so that the minimum value of
$\Pxa$ across all ancilla assignments is 0 when x is a model and 
$\ge g_{min}$ when x is not a model.}

\begin{IGNORE}
%% GIA? SCRITTO DOPO
This can be written as:
%
\begin{eqnarray}
\label{eq:encoding1}
\exists \ts.\forall \xs.\ 
\left [ 
\begin{array}{ll}
{(\pos\Fx \imp \forall \as. (\Pxa\ge 0 ))\  \wedge}\\
(\pos\Fx \imp \exists \as. (\Pxa=0 ))\  \wedge\\
(\neg\Fx \imp \forall \as. (\Pxa\ge g_{min} ))\  
\end{array}
\right ]
\end{eqnarray}
\end{IGNORE}

\begin{figure}[t]
\subfigure[\label{fig:mappings_xor}$x_3 \iff (x_1 \oplus x_2)$ with three ancillas
%(Ex.~\ref{ex:xor1}).
]%
{\includegraphics[width=0.21\columnwidth]{xorgraph.pdf}\ \ \ \ \ 
}
\subfigure[\label{fig:mappings_and}$x_3 \iff (x_1 \wedge x_2)$ with one ancilla.]%
{\includegraphics[width=0.21\columnwidth]{andgraph.pdf}}
\caption{\label{fig:mappings} Mappings within the Chimera HW graph.}
\end{figure}


\begin{example}
\label{ex:xor1}
  The xor function of Example~\ref{es:examplexor} 
  can be encoded with three ancillas $a_1, a_2, a_3$ as:
  $
  \Pxa = \Pxa = 5 + x_3 + a_2 - a_3 + x_1 a_1  - x_1 a_2 - x_1 a_3 - x_2 a_1 - x_2 a_2 
  - x_2 a_3 + x_3 a_2 - x_3 a_3
  $, which is mapped as in figure ~\ref{fig:mappings_xor}.
%%   \begin{equation*}
%%     \begin{split}
%%       \Pxa = 4.375 + 0.125 x_1 - 0.5 x_2 + x_3 - 0.5 a_1 + 0.75 a_2 \\+ 0.375 a_3
%%   -0.5 x_1 a_1 - x_1 a_2 + 0.375 x_1 a_3 + 0.5 x_2 a_1 \\ - 0.5 x_2 a_2 - x_2 a_3
%%   - x_3 a_1 + x_3 a_2 - x_3 a_3
%% \end{split}
%% \end{equation*}
%% Which can be fit on a Chimera tile in the following way:
%
%% \centering
%% \includegraphics[width=0.2\columnwidth]{xorgraph.pdf}
\end{example}
%
\begin{example}
The and funcyion of Example~\ref{es:exampleand}
can be encoded with one ancilla $a$ as:
$\Pxa =  \frac{9}{2} - \frac{1}{2} x_1 - \frac{1}{2} x_2 + x_3 + \frac{1}{2}
x_1 x_2 - x_1 x_3 - x_2a - x_3a $, which is mapped as in figure ~\ref{fig:mappings_and}.
%% \begin{center}
%% \includegraphics[width=0.2\columnwidth]{andgraph.pdf}
%% \end{center}
\end{example}

This formula is $\exists\forall\exists$-quantified. For this reason, finding the smallest conversion is a
problem in the $\Sigma_3^P$ complexity class; it is actually harder than the
original SAT problem we started with. Direct encoding of an input problem is not
viable for direct conversion of problems.
For smaller problems we can use a SMT solver to find a solution by expanding the quantifiers through
Shannon expansion \cite{rsebanote}. In this way though, the size
of expanded formula increases exponentially and thus become impractical for
bigger encodings.


==> qa_detail.tex <==
%\subsubsection{Detail about QA and D-Wave QPU}
%The number of qubits and their connectivity in current QA hardware restrict the Ising models that can be programmed. 
Practical QA systems are physical, analog
devices, subject to engineering limitations. Most importantly, the D-Wave
2000Q  offers  sparse connectivity between
variables. The connectivity graph $G$ of current D-Wave
processors is shown in Figure~\ref{chimera}, and is called the
\emph{Chimera} graph. 
%\RSCOMMENT{Content moved from caption of fig~3 to here.}
This topology consists of a lattice of strongly-connected
    components of 8 qubits, called \emph{tiles}. Each tile consists of
    a complete bipartite graph between two sets of four qubits. One
    set, the ``vertical" set, is connected to the tiles above and
    below; the other set, the ``horizontal" set, is connected to the
    tiles to the left and to the right. Notice that each qubit is
    connected with at most six other qubits. In other words, each
    variable $z_i$ in the Ising model \eqref{eq:isingmodel} has at
    most $6$ non-zero $\DWcoupij{}$ interactions with other
    variables.

Beyond that, programming requires an understanding of how the choice of Ising model affects hardware performance. Among the most relevant factors are:
\begin{itemize}
\item \emph{Energy gaps}. In practice, QA hardware does not always return a solution $\zs ^*$ with minimum energy $E(\zs^*)$ in \eqref{eq:isingmodel}. A better (though still inaccurate \cite{amin15quasistatic,kulchytskyy2016qbm,raymond2016warming}) approximation of the hardware's behaviour is Boltzmann sampling: state $\zs$ is returned with probability
\begin{equation}
p(\zs) \sim e^{-\beta E(\zs)}
\label{eqn:boltzmann}
\end{equation}
for some fixed inverse temperature $\beta > 0$. From \eqref{eqn:boltzmann}, we see that a larger energy gap $g_{min}$ between ground and excited states leads to a higher probability of an optimal solution, as a ground state is $e^{\beta g_{min}}$ times more likely than a first excited state. 
\item \emph{Intrinsic control error}. Due to various engineering limitations and sources of environmental noise, the Ising model $[h,J]$ implemented in QA hardware is not exactly the one programmed by the user. The D-Wave 2000Q
system currently requires $\DWbiasi \in [-2,2]$ and
$\DWcoupij{} \in [-1,1]$. A reasonable model of error is that each specified $h_i$ and $J_{ij}$ is subject to Gaussian noise with standard deviation $3\%$ and $2\%$ respectively. As a result, all other things being equal, Ising models with fewer qubits are preferable because they are subject to less noise.
\item \emph{Freeze-out}. 
Because of the limited connectivity of the processor, we often use several physical qubits to represent a single logical variable. We call those qubits a \emph{chain} and discuss how to implement them in Section \ref{sec:problems_embedding}. However, the \emph{quantum tunnelling} effect on which QA is based is diminished for chains \cite{lanting10tunneling}. A chain of many qubits is likely to become frozen in a particular configuration earlier in annealing than a chain of few qubits or a single qubit, and this early freeze-out reduces the hardware's ability to find global minima. This effect can be partially mitigated by constructing Ising models with chains as small as possible.
\end{itemize}


==> sv_macros.tex <==
\makeatletter
\pgfkeys{/pgf/.cd,
	parallelepiped offset x/.initial=2mm,
	parallelepiped offset y/.initial=2mm
}
\pgfdeclareshape{parallelepiped}
{
	\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
	\inheritanchorborder[from=rectangle]
	\inheritanchor[from=rectangle]{north}
	\inheritanchor[from=rectangle]{north west}
	\inheritanchor[from=rectangle]{north east}
	\inheritanchor[from=rectangle]{center}
	\inheritanchor[from=rectangle]{west}
	\inheritanchor[from=rectangle]{east}
	\inheritanchor[from=rectangle]{mid}
	\inheritanchor[from=rectangle]{mid west}
	\inheritanchor[from=rectangle]{mid east}
	\inheritanchor[from=rectangle]{base}
	\inheritanchor[from=rectangle]{base west}
	\inheritanchor[from=rectangle]{base east}
	\inheritanchor[from=rectangle]{south}
	\inheritanchor[from=rectangle]{south west}
	\inheritanchor[from=rectangle]{south east}
	\backgroundpath{
		% store lower right in xa/ya and upper right in xb/yb
		\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
		\pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/parallelepiped offset x}}
		\pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/parallelepiped offset y}}
		\def\ppd@offset{\pgfpoint{\pgfutil@tempdima}{\pgfutil@tempdimb}}
		\pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
		\pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
		\pgfpathclose
		\pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@ya}}{\ppd@offset}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\ppd@offset}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xa}{\pgf@yb}}{\ppd@offset}}
		\pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
		\pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\ppd@offset}}
	}
}
%\makeatother
%\DeclareUnicodeCharacter{0301}{\'}

